Cascading Bandits for Large-Scale Recommendation Problems

Most recommender systems recommend a list of items. The user examines the list, from the first item to the last, and often chooses the first attractive item and does not examine the rest. This type of user behavior can be modeled by the cascade model. In this work, we study cascading bandits, an online learning variant of the cascade model where the goal is to recommend $K$ most attractive items from a large set of $L$ candidate items. We propose two algorithms for solving this problem, which are based on the idea of linear generalization. The key idea in our solutions is that we learn a predictor of the attraction probabilities of items from their features, as opposing to learning the attraction probability of each item independently as in the existing work. This results in practical learning algorithms whose regret does not depend on the number of items $L$. We bound the regret of one algorithm and comprehensively evaluate the other on a range of recommendation problems. The algorithm performs well and outperforms all baselines.

==> Rosemary.tex <==
%!TEX root = Paper.tex

\subsection{Experiment Rosemary}
\label{sec:experiment Rosemary}

\todos{Need to revise the title for this subsection}

\subsubsection{Dataset}
\label{sec:Dataset Rosemary}
In our experiment, we evaluate our feature learning method on Yahoo! music dataset. The dataset contains a large sample of Yahoo! music user ratings of music artists. There are over 11 million ratings for 98k artist by over 1 million users. Each entry in the ratings contains an anonymous user ID, an artist ID and a corresponding rating. 
We would like to learn a feature representation that best presents our artist ratings. Ideally, the more similar the music artist, the closer they should be in the feature space. 

We pick the ratings from the top 1000 users to rate the most rated 256 and 16 artist, and represent the artist as a vector consisting of user ratings. For example, artist A is given a rating of 90 by user A and rating of 50 by user B. If the rating is above 50/100 from the user, we count it as a rating of 1, otherwise, it would be counted as 0.

\subsubsection{Results}
Bababala




